DeepLandscape: Adversarial Modeling of Landscape Video

We build a new model of landscape videos that can be trained on a mixture of static landscape images as well as landscape animations. Our architecture extends StyleGAN model by augmenting it with parts that allow to model dynamic changes in a scene. Once trained, our model can be used to generate realistic time-lapse landscape videos with moving objects and time-of-the-day changes. Furthermore, by fitting the learned models to a static landscape image, the latter can be reenacted in a realistic way. We propose simple but necessary modifications to StyleGAN inversion procedure, which lead to in-domain latent codes and allow to manipulate real images. Quantitative comparisons and user studies suggest that our model produces more compelling animations of given photographs than previously proposed methods. The results of our approach including comparisons with prior art can be seen in supplementary materials and on the project page https://saic-mdal.github.io/deep-landscape

==> tables/abl_gen.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

% OLD 
% \begin{table}[]
% \begin{tabular}{@{}l|l|l|l|l|l|l@{}}
% Metric & \begin{tabular}[c]{@{}l@{}}Vanila \\ (only video)\end{tabular} & \begin{tabular}[c]{@{}l@{}}+ frame\_discr\\ + decay\end{tabular} & + two noises & +z3       & +shift\_crop       & \begin{tabular}[c]{@{}l@{}}+nfd\_freq\_01\\ +nfd\_freq\_03\end{tabular} \\ \midrule \hline
% FID    & 58.587675 & \begin{tabular}[c]{@{}l@{}}-\\ 67.284264\end{tabular}            & 65.639667    & 66.566888 & \textbf{65.372986} & \\ \midrule \hline
% LPIPS  & \textbf{0.048975} & \begin{tabular}[c]{@{}l@{}}-\\ 0.057621\end{tabular} & 0.064572 & 0.055559 & 0.053071           & \\ \midrule \hline
% SSIM   & 0.775965 & \begin{tabular}[c]{@{}l@{}}-\\ 0.806356\end{tabular} & 0.831802 & 0.856853 & \textbf{0.878411}  &
% \end{tabular}
% \end{table}


% NEW
\begin{table}[]
\begin{tabular}{@{}l|l|l|l|l|l|l@{}}
Metric & \begin{tabular}[c]{@{}l@{}}Vanila \\ (only video)\end{tabular} & + frame\_discr and decay & + two noises & +z3       & +shift\_crop \\ \midrule \hline
FID & \textbf{48.395962} & 55.918984 & 55.151618 & 54.384753 & 56.130700 & \\ \midrule \hline
LPIPS & \textbf{0.048975} & 0.064456 & 0.073446 & 0.064517 & 0.062163 & \\ \midrule \hline
SSIM & 0.809567 & 0.846145 & 0.854497 & 0.879259 & \textbf{0.883567}  &
\end{tabular}
\end{table}

==> tables/fid.tex <==
\begin{table}[]
\centering
\caption{Comparing quality difference between input image and generated frames}
\begin{tabular}{l|l}
Method                                  & $Mean_n$ FID($I_0$, $\widehat{I_n}$) \\ \hline
Shaham et al., 2018 & 69.0035 \\ \hline
Endo et al., 2019 \\ w/ interpolation & 69.3604 \\ \hline
Endo et. al. 2019 \\ w/out interpolation & 54.8452 \\ \hline
Ours, eoifs & 52.3513 \\ \hline
Ours, eoif & \textbf{45.3652} \\ \hline
Original Videos ($\hat{I_n} = I_n$)     & 28.89                  \\ \hline
\end{tabular}
\end{table}


==> tables/fvd.tex <==
\begin{table}[]
\begin{tabular}{l|l|l|l}
\textbf{Method}                                  & FVD$_{min}\downarrow$& PD$_{mean}\downarrow$&
FID$_{mean}\downarrow$
\\ \hline
SG & 210.658 & 0.2415 & 69.1191 \\ 
\hline
AL & 275.727 & 0.2708 & 69.4339
\\ \hline
AL w/out interpolation & 162.01 & 0.2327 &
54.9867
\\ \hline
Ours, eoifs & 161.044 & 0.2393 & 52.4668
\\ \hline
Ours, eoif & \textbf{149.891} & \textbf{0.2273} & \textbf{45.5355}
\\ \hline 
\end{tabular}
\end{table}

==> tables/quantitive.tex <==
\begin{table}[]
\begin{tabular}{|l|l|l|l|}
\hline
Model             & Dataset                                                & \multicolumn{1}{r|}{FVD} & SIFID \\ \hline
SinGAN            & \begin{tabular}[c]{@{}l@{}}Urban\\ Nature \\ Clouds\end{tabular} &                          &       \\ \hline
Endo et. al. 2019 & \begin{tabular}[c]{@{}l@{}}Urban\\ Nature \\ Clouds\end{tabular} &                          &       \\ \hline
Ours              & \begin{tabular}[c]{@{}l@{}}Urban\\ Nature \\ Clouds \end{tabular} &                          &       \\ \hline
\end{tabular}
\end{table}

==> tables/user_study_fake_vs_real.tex <==
\begin{table}[]
\begin{tabular}{l|l|l|l}
\textbf{Method}     & Fooling Rate 
\\ \hline
AL (+ style) & 0.246377 
\\ \hline
SG & 0.376812
\\ \hline
Sunthetic & 0.417391
\\ \hline
AL (no int) &  0.541063
\\ \hline
Real &   0.594203
\\ \hline
Ours (EOIFS) & 0.621256 
\\ \hline 
Ours (EOIF) & \textbf{0.630918}
\\ \hline 
\end{tabular}
\end{table}



% al_st                                      0.246377
% sg                                         0.376812
% abl_two_noise_z3_shift_crop_nfd_freq_01    0.388406
% abl_two_noise_z3_shift_crop_decay_         0.417391
% al                                         0.541063
% gt                                         0.594203
% EOIFS                                      0.621256
% EOIF                                       0.630918
